Are we describing the same sound? An analysis of word embedding spaces of expressive piano performance

Semantic embeddings play a crucial role in natural language-based information retrieval. Embedding models represent words and contexts as vectors whose spatial configuration is derived from the distribution of words in large text corpora. While such representations are generally very powerful, they might fail to account for fine-grained domain-specific nuances. In this article, we investigate this uncertainty for the domain of characterizations of expressive piano performance. Using a music research dataset of free text performance characterizations and a follow-up study sorting the annotations into clusters, we derive a ground truth for a domain-specific semantic similarity structure. We test five embedding models and their similarity structure for correspondence with the ground truth. We further assess the effects of contextualizing prompts, hubness reduction, cross-modal similarity, and k-means clustering. The quality of embedding models shows great variability with respect to this task; more general models perform better than domain-adapted ones and the best model configurations reach human-level agreement.

==> tables/table_overlap.tex <==
\begin{tabular}{l|lclc|lcc}
\toprule
 Ref & P1 in P2: & 0.62     &P2 in P1:&0.65&&&    \\
   \midrule
   \textbf{Model} & \multicolumn{2}{l}{\textbf{Overlap v P1}} &  
   \multicolumn{2}{l}{\textbf{Overlap v P2}} & 
   \multicolumn{3}{l}{\textbf{WvB Distance Ratio}}   \\
   \midrule
   ADA & 0.55 &    0.58 &    0.48 &    0.43 &    1.69 &    1.96 &    1.53\\
   CLAP & 0.52 &    0.51 &    0.47 &    0.46 &    1.62 &    2.00 &    1.04\\
   GTE & 0.59 &    0.59 &    0.53 &    0.52 &    1.72 &    1.97 &    1.50\\
  BGE &  0.51 &    0.53 &    0.53 &    0.48 &    1.71 &    1.99 &    1.35\\
  GT &  0.66 &    0.70 &    0.66 &    0.70 &    1.10 &    1.14 &    1.00\\
  RB &  0.39 &    0.41 &    0.40 &    0.39 &    2.08 &    2.57 &    0.89\\
\bottomrule
\end{tabular}

    
    
    
    
    
